FedAdapter: Efficient Federated Learning for Modern NLP

Transformer-based pre-trained models have revolutionized NLP for superior performance and generality. Fine-tuning pre-trained models for downstream tasks often requires private data, for which federated learning is the de-facto approach (i.e., FedNLP). However, our measurements show that FedNLP is prohibitively slow due to the large model sizes and the resultant high network/computation cost. Towards practical FedNLP, we identify as the key building blocks adapters, small bottleneck modules inserted at a variety of model layers. A key challenge is to properly configure the depth and width of adapters, to which the training speed and efficiency is highly sensitive. No silver-bullet configuration exists: the optimal choice varies across downstream NLP tasks, desired model accuracy, and mobile resources. To automate adapter configuration, we propose FedAdapter, a framework that enhances the existing FedNLP with two novel designs. First, FedAdapter progressively upgrades the adapter configuration throughout a training session; the principle is to quickly learn shallow knowledge by only training fewer and smaller adapters at the model's top layers, and incrementally learn deep knowledge by incorporating deeper and larger adapters. Second, FedAdapter continuously profiles future adapter configurations by allocating participant devices to trial groups. Extensive experiments show that FedAdapter can reduce FedNLP's model convergence delay to no more than several hours, which is up to 155.5$\times$ faster compared to vanilla FedNLP and 48$\times$ faster compared to strong baselines.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

BIBLATEXFILES= $(wildcard *.bbx) $(wildcard *.cbx) $(wildcard *.dbx) $(wildcard *.lbx)
SAMPLEBIBLATEXFILES=$(patsubst %,samples/%,$(BIBLATEXFILES))

all:  ${PDF} ALLSAMPLES

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES: $(SAMPLEBIBLATEXFILES)
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/abbrev.bib: ACM-Reference-Format.bst
	perl -pe 's/MACRO ({[^}]*}) *\n/MACRO \1/' ACM-Reference-Format.bst \
	| grep MACRO | sed 's/MACRO {/@STRING{/' \
	| sed 's/}  *{/ = /' > samples/abbrev.bib 


samples/%.bbx: %.bbx
samples/%.cbx: %.cbx
samples/%.dbx: %.dbx
samples/%.lbx: %.lbx

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-sigconf-biblatex.pdf: samples/sample-sigconf-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-acmsmall-biblatex.pdf: samples/sample-acmsmall-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done

samples/sample-acmcp.pdf: samples/acm-jdslogo.png

.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut \
	samples/acm-jdslogo.png \
	samples/*.run.xml samples/*.bcf $(SAMPLEBIBLATEXFILES)


clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

# distros
distros: all docclean
	zip -r acm-distro.zip  \
	acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.* \
	--exclude samples/sample-acmengage*
	zip -r acmengage-distro.zip samples/sample-acmengage* \
	samples/*.bib \
	acmart.pdf acmguide.pdf  *.cls ACM-Reference-Format.*


.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

Version 1.89a  Added version info to .bst

Version 1.89   Bug fixes
	       Redesign of ACMCP
	       New positioning of badges
	       New journals: PACMMOD, TOPML

Version 1.88   New ISSNs
	       Documentation updates
	       New journal:  PACMNET

Version 1.87   CC license is allowed for non-acm documents and ACM Engage
	       documents only
	       New format acmcp for the cover page
	       New journals: JATS, ACMJCSS, TORS
	       Bug fixes

Version 1.86.  Empty country in affiliation now produces an error
               Bug fixes
	       New samples for acmengage

Version 1.85.  Bug fixes
	       Added support for Creative Commons licenses (requires
	       doclicense images)
	       New journals
	       New format acmengage for ACM Engage CSEdu course materials 

Version 1.84   Support for BibLaTeX rewritten (thanks to
	       Roberto Di Cosmo and Kartik Singhal)
	       Corrected German translation (thanks to Dirk Beyer)
	       New journals

Version 1.83   Support for multilanguage papers
	       ISSN changes for some journals

Version 1.82   Bug fixes.
	       New command \anon for anonymization of short strings.
	       Documentation update.

Version 1.81   Bug fixes
	       New bib field distinctURL to print URL even if doi is present.
	       Reworded samples

Version 1.80   New journals: DLT, FAC

Version 1.79   Fixed pages with index
	       (https://github.com/borisveytsman/acmart/issues/440)
	       Updated information for TAP, TCPS, TEAC

Version 1.78   Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.

Version 1.77   Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.76   Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.75   Omitted \country now produces error.
	       Added \AtBeginMaketitle

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations.  The absence of them produces a warning

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.63a   Moved TQUANT to TQC

Version 1.63	New journals: TQUANT, FACMP

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.52    Another rewording of licenses

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.49    New jorunal:  DTRAP

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.47    New journal: THRI

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.43    Bug fixes

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.41    Rearranged bib files
                Added new badges

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.39    Added \authornotemark commmand

Version 1.38    Increase default font size for SIGPLAN

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

Version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

Version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

Version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

Version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

Version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

Version 1.28    Bug fixes: natbib=false now behaves correctly.

Version 1.27    Bug fixes

Version 1.26    Bug fixes

Version 1.25    Updated PACMPL journal option.

Version 1.24    Added IMWUT journal option.

Version 1.23    Added PACM PL journal option.

Version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

Version 1.21    Bibliography changes: added arXiv, some cleanup

Version 1.20    Bug fixes, documentation updates

Version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

Version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.


Version 1.17    Formatting changes for margins and lists.  Bug fixes.

Version 1.16    Formatting changes for headers and footers.

Version 1.15    New structured affiliation command.
                New commands for acknowledgements.

Version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

Version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

Version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

Version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

Version 1.10    Bug fixes

Version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

Version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes


==> alg-backup.tex <==
\begin{algorithm}
    \caption{Backup for VFL}%算法名字
    %\LinesNumbered %要求显示行号
    \KwIn{dataset $x_{i}^{A_{k}}$, dataset $x_{i}^{B}$, backups $\beta$  }%输入参数
    \KwOut{Model parameters $\Theta_{A_{k}}, \Theta_{B}(k=1,2..K)$}%输出
    Party $A_{k},B$ initialize $\Theta_{A_{k}}, \Theta_{B}$;
    
    \For{each iteration $j=1,2 \ldots$}{
        Parallel: Host(j),Guest(j)
    }
    Host(j):

    \For{k=1,2..K in parallel}{
        $A_{k}$ computes $u_{i}^{A_{k}}$, and send $[[u_{i}^{A_{k}}]], [[\Theta_{A_{k}}^{2}]]$ to B

        Get $[[d_{i}]]$ from $B$

        Updata $\Theta_{A_{k}}$ with (\ref{algorithm-gradient}) (\ref{algorithm-update})
    }

    Guest(j):

    \eIf{$\left|[[u_{i}^{A_{k}}]]\right|< K-\beta$}{
        Waiting for $u_{i}^{A_{k}}$ from $A_{k}$
    }{
        B computes $d_{i}$ with (\ref{algorithm-backup2}) and sends $[[d_{i}]]$ to $A_{k}$
    }
    Updata $\Theta_{B}$ with (\ref{algorithm-gradient}) (\ref{algorithm-update})
    \label{algo-1}
\end{algorithm}


==> alg-cache.tex <==
\begin{algorithm}
	\footnotesize
	\SetAlgoNoEnd
  \SetKwData{Left}{left}\SetKwData{This}{this}\SetKwData{Up}{up}
  \SetKwFunction{MIN}{MIN}\SetKwFunction{MAX}{MAX}\SetKwFunction{LENGTH}{LENGTH}
  \SetKwInOut{Input}{input}\SetKwInOut{Output}{output}\SetKwInOut{Variable}{Variable}

  \Input{
      Finetuning depth, $d_{prev}=-1$;\\
      Overall depth, $D$.
    }
  % \Variable{
  %   Latency of load layer $i$ \quad $T_i$ for $0 \leq i \leq N$\; \\
  %   Latency of execution \quad $T_f$\; \\
  %   Cold-infer. time with kernels' combination $k$ \quad $T_{cold}^k$\; \\
  %   Total time of $Q_j$ \quad $sum_j$
  %   }

  \Output{
      Fine-tuned adapter weights, $\Theta_{i}(i=1,2..)$.
      % $Q_b$\;   
    }
  \BlankLine
  
  Client(k):\\
  \While{Available}
  {   
      \eIf{Chosen}{
          $d^{\prime}=\max (d_{\text {prev }}, d_{\text {prev }+1}, \ldots, d_{\text {now }})$;\\
          \eIf{$d^{\prime}>d_{p r e v}$}{
              Do the normal finetuning; \\
              Extracts the output of the first $D-d_{\text {prev }}$ transformer layers and store them  in local storage.
              }{
              Load the output of layer $d_{\text {split }}$ from disk;\\
              Feed it into the training process without starting from scratch.
              }
      }{
      Idle.
      }
  }
  \caption{On-device Activations Caching}\label{alg:cache}
\end{algorithm}

==> alg-pipelined.tex <==
\begin{algorithm}
	\footnotesize
	\SetAlgoNoEnd
  \SetKwData{Left}{left}\SetKwData{This}{this}\SetKwData{Up}{up}
  \SetKwFunction{MIN}{MIN}\SetKwFunction{MAX}{MAX}\SetKwFunction{LENGTH}{LENGTH}
  \SetKwInOut{Input}{input}\SetKwInOut{Output}{output}\SetKwInOut{Variable}{Variable}

  \Input{
      Number of little cores, $M_l$; \\
      Number of layers, $N$ \; \\
      % Layers \quad $L_i$ for $0 \leq i \leq N$\; \\
      Sets of candidate kernels' combination, $K$;\\
      operation $r_i$, $w_i$, $e_i$ ($i\in\{1,2,...,N\}$). 
    }
  % \Variable{
  %   Latency of load layer $i$ \quad $T_i$ for $0 \leq i \leq N$\; \\
  %   Latency of execution \quad $T_f$\; \\
  %   Cold-infer. time with kernels' combination $k$ \quad $T_{cold}^k$\; \\
  %   Total time of $Q_j$ \quad $sum_j$
  %   }

  \Output{
      Combination of selected kernels, $K_c$;\\
      The list of operation running on little core $j$, \\$Q_j$ ( $j\in\{1,2,...,M_l\}$);\\
      The list of operation running on BIG cores, $Q_0$.
      % $Q_b$\;   
    }
  \BlankLine
  
  % Kernel selection and whether Bypassed weights transformation; \\
  Filter out the kernel candidates that exhibit no faster operation; \\
  \ForEach{combination $k=\{<r_i,w_i,e_i>|i=1,2,...N\}$ ($k\in K$)}
{    % Get $T_i$ for $0 \leq i \leq N$ and $T_f$; \\
  Initialize $Q_0$: Insert the operation $r_1$, $w_1$ and all $e_i$ of $k$ into the BIG cores sequentially, s=2;\\
  Initialize the execution time of the operations on core $j$: $T_{Q_j}=0, ~j\in \{0,1,...,M_l\}$;\\
  %Initialize $Q_j$ (j=1,..,M_l): schedule $r_i$, $w_i$ (i=2,..,N) to different small cores sequentially;\\
  Update the execution time of operation $o$ on little cores $t_o^{\rm l}$ and BIG cores $t_o^{\rm b}$; \\
  \While{$\left|\max\limits_{1 \leq j  \leq M_l} T_{Q_j} - T_{Q_0}\right| \textgreater  \varepsilon$ or $T_{Q_j}=0, ~(j\in \{0,1,...,M_l\})$
  }
  {
  % \While{\MAX{$sum$}-($T_f$ + $T_{Q_b}$) $\leq  \varepsilon$}{
      \uIf{$\max\limits_{1 \leq j \leq M_l} T_{Q_j} \textgreater  T_{Q_0}$}{
        \For{$i\leftarrow s$ \KwTo $N$}{
            \uIf{$(t_{r_i}^{\rm b}+ t_{w_i}^{\rm b}) +(t_{r_i}^{\rm l}+ t_{w_i}^{\rm l}) < \max\limits_{ 1 \leq j  \leq M_l} T_{Q_j} -T_{Q_0}$}{
                Insert $r_i$, $w_i$ into $Q_0$ header, $s := i$ ; \\
                \textbf{break};
            }
        }
      }
      % \For{$i\leftarrow S+1$ \KwTo $M_l+S+1$}{
      %   Insert $L_i$ into $Q_i$
      % }
      % \For{$i\leftarrow M_l+S+2$ \KwTo $N$}{
      %   \lFor{$j\leftarrow 1$ \KwTo $M_l$}{
      %       $sum_j$ := $\Sigma (T_a | L_a \in Q_j)$
      %   }
      %   \For{$j\leftarrow 1$ \KwTo $M_l$}{
      %       \uIf{$sum_j$ == \MIN{$sum$}}{
      %           Insert $L_i$ into $Q_j$;
      %       }
      %   }
      % }
      %Initialize $Q_1$ \textasciitilde $Q_{M_l}$ with operation except those in $Q_0$\\
      Initialize $Q_j~ (j=1,..,M_l)$: schedule $r_i$, $w_i$ ($i=s+1,..,N$) to different little cores sequentially;\\
      \While{$\max\limits_{1 \leq j \leq M_l} T_{Q_j} - \min\limits_{1 \leq j \leq M_l} T_{Q_j} \textgreater \varepsilon$}{
        % \lFor{$j\leftarrow 1$ \KwTo $M_l$}{
        %     $sum_j$ := $\Sigma (T_a | L_a \in Q_j)$
        % }
        $j_{\rm max} := \arg \max\limits_{1 \leq j \leq M_l} T_{Q_j}$ \\
        $j_{\rm min} := \arg \min\limits_{1 \leq j \leq M_l} T_{Q_j}$ \\
        % \For{$j\leftarrow 1$ \KwTo $M_l$}{
        %     \lIf{$sum_j$ == \MIN{$sum$}}{
        %         $Q_{min} := Q_j$
        %     }
        %     \lIf{$sum_j$ == \MAX{$sum$}}{
        %         $Q_{max} := Q_j$
        %     }
        % }
        % $diff := T_{i_{max}} -  T_{i_{min}}$ \\
        Sort operation in $Q_{j_{max}}$ descendingly according to the execution time as $Q_{sort}$;\\
        \ForEach{operation $(r,w)$ in $Q_{sort}$}{
          \uIf{$t_r^{\rm l}+ t_w^{\rm l} < \frac{T_{Q_{j_{\rm max}}}-T_{Q_{j_{\rm min}}}}{2}$}{
            Move ($r$, $w$) from $Q_{i_{max}}$ to $Q_{i_{min}}$; \\
                     }
        }
        % Get $T_i$ for $0 \leq i \leq N$ and $T_f$ with $k$; \\
       % Update $t(f,i)$, $f \in Q_i$, $0 \leq i  \leq M_l$ ; \\
        %\For{$j=0:M_l$}{
        %  $T_{Q_i} := \sum t(f, i)$, $f \in Q_i$ \\
        %}
        Compute $T_{Q_j}$ ($j=0,1,..,M_l$);       
      }
  }
  Compute the completion time of kernel combination $k$, $T_{cold}^k$; \\
  }
  $K_c$ = $\arg \min\limits_k(T_{cold}^k)$
  \caption{Our kernel scheduler}\label{alg:scheduler}
\end{algorithm}

==> alg-trial_bk.tex <==
\begin{algorithm}
	\footnotesize
	\SetAlgoNoEnd
  \SetKwProg{Fn}{Function}{ is}{end}
  \SetKwData{Left}{left}\SetKwData{This}{this}\SetKwData{Up}{up}
  \SetKwFunction{MIN}{MIN}\SetKwFunction{MAX}{MAX}\SetKwFunction{LENGTH}{LENGTH}
  \SetKwInOut{Input}{input}\SetKwInOut{Output}{output}\SetKwInOut{Variable}{Variable}

  \Input{
      % Pre-trained model, $\Theta$;\\
      Trial duration, $T$;\\
      Start-up depth and width, $D_{0}$ and $W_{0}$;\\
      Step of depth and width, $S_d$ and $S_w$.
    }

  \Output{
      Fine-tuned adapter weights, $\Theta_{i}~(i=1,2 \ldots)$.
      % $Q_b$\;   
    }
  \BlankLine
  
  
  Server selects $3N$ clients shuffuled into 3 groups: $Trial_{0}$, $Trial_{1}$, $Trial_{2}$;\\
  Dispatch(0);\\
  \For{each iteration $i=1,2 \ldots$}{
      Parallel: $Trial_{k}(i)$ ($k=0,1,2$);\\
      Server(i)
        
  }

  \Fn{$Trial_{k}(i)$($k=0,1,2$):}{
  

  \ForEach{Client(n) in $Trial_{k}(i)$ ($n=0,1,..,N-1$)}{
    Receive global adapter $\Theta_{i-1}^{k}$ from Server;\\
    Train and update local adapter $\Theta_{i}^{k}(n)$ inserted into pre-trained models through activation caching.; \\
    Send updated adapter $\Theta_{i}^{k}(n)$ to Server.
  }
  }
  
  \Fn{Server(i):}{

  Recieve $\Theta^{k}_{i}(n)$ from $Trial_{k}$;\\
  Fedavg aggregation: $\Theta^{k}_{i}=\frac{\sum^{N-1}_{n=0}\Theta^{k}_{i}(n)}{n}$;\\
  Select $3N$ new clients shuffuled into 3 groups: $Trial_{0}$, $Trial_{1}$, $Trial_{2}$;\\
  \eIf{Runtime $t<T$}
  { 
    $D_{i}=D_{i-1}, W_{i}=W_{i-1}$; \\
    Send the aggregated model $\Theta_{i}^{k}$ to selected clients.
  }{
    Compare evluation metrics under different $\Theta^{k}_{i}$;\\
    Set the winner track as $\Theta_{i}$;\\
    Set the winner setting as $D_{i}, W_{i}$;\\
    Dispatch(i);\\
    Reinitialize runtime = 0
  }
  }

  \Fn{Dispatch(i):}{

  \eIf{i=0}
  {
    $F$($D$,$W$): Initial $\Theta_{0}$ with $D$, $W$
  }{
    $F$($D$,$W$): Inherit $\Theta_{i}$ from the winner track with $D$, $W$
  }
  
  $\Theta_{i}^{0}$=$F$($D_{i}$,$W_{i}$);\\
  $\Theta_{i}^{1}$=$F$($D_{i}+S_{d}$,$W_{i}$);\\
  $\Theta_{i}^{2}$=$F$($D_{i}$,$W_{i}+S_{w}$);\\
  Sends $\Theta_{i}^{0}$, $\Theta_{i}^{1}$, $\Theta_{i}^{2}$ to $Trial_{0}$, $Trial_{1}$, $Trial_{2}$ seperately\;
  }

  \caption{Our Online Configurator}\label{alg:trial}
\end{algorithm}

==> fig-adapter-tradeoffs.tex <==
\begin{figure}[t]
	\centering
	\begin{minipage}[b]{0.24\textwidth}
		\includegraphics[width=1.0\textwidth]{figs/design-adapter-tradeoffs.pdf}
		\subcaption{Dataset1}
	\end{minipage}
	~
	\begin{minipage}[b]{0.24\textwidth}
		\includegraphics[width=1.0\textwidth]{figs/design-adapter-tradeoffs.pdf}
		\subcaption{Dataset2}
	\end{minipage}
	\caption{The tradeoffs opened by adapters between model accuracy and trainable parameter number.}
	% \caption{The performance breakdown of computation and communication time. Note that y-axis is logarithmic.}
	\label{fig:design-adapter-tradeoffs}
\end{figure}

==> fig-design-adapter-width.tex <==
\begin{figure}[t]
	\centering
	 \includegraphics[width=0.48\textwidth]{figs/design-adapter-width.png}
	\caption{Validation set accuracy versus number of trained parameters for three methods: (i) Adapter tuning with an adapter sizes $2^{n}$ for $n=0 \ldots 9$ (orange). (ii) Fine-tuning the top $k$ layers for $k=1 \ldots 12$ (blue). (iii) Tuning the layer normalization parameters only (green). Error bars indicate $\pm 1$ s.e.m. across three random seeds. \mwx{fig copied.} \textbf{If not our figure, better not to show it. Btw, how is adapter size defined?}} 
	\label{fig:design-adapter-width}
\end{figure}


==> fig-design-cache-perf.tex <==
% \begin{figure}[t]
% 	\centering
% 	\begin{minipage}[b]{0.23\textwidth}
% 		\includegraphics[width=1\textwidth]{figs/design-cache-workflow.pdf}
% 		\caption{The overall workflow of activation caching.} 
% 	\end{minipage}
% 	\label{fig:design-cache-workflow}
% 	~
% 	\begin{minipage}[b]{0.23\textwidth}
% 		\includegraphics[width=1\textwidth]{figs/design-cache-perf.pdf}
% 		\caption{A micro experiment to compare the per-batch training cost with and without activation caching.} 
% 		\label{fig:design-cache-perf}
% 	\end{minipage}
% \end{figure}

% \begin{figure}[t]
% 	\centering
% 	\includegraphics[width=0.48\textwidth]{figs/design-cache-workflow.pdf}
% 		\caption{The overall workflow of activation caching.} 
% 		\label{fig:design-cache-workflow}
% \end{figure}

\begin{figure}[t]
	\centering
	\includegraphics[width=0.24\textwidth]{figs/design-cache-perf.pdf}
	\vspace{-10pt}
		\caption{Per-batch training time with and without activation caching. Model: DistilBERT. Device: Jetson TX2.} 
		\vspace{-10pt}
		\label{fig:design-cache-perf}
\end{figure}


==> fig-design-cache-workflow.tex <==
\begin{figure}[t]
	\centering
	 \includegraphics[width=0.48\textwidth]{figs/design-cache-workflow.pdf}
	\caption{The overall workflow of activation caching.} 
	\label{fig:design-cache-workflow}
\end{figure}


==> fig-eval-ablation-adapter.tex <==
\begin{figure}[t]
	\centering
	\includegraphics[width=0.48\textwidth]{figs/eval-ablation-adapter.pdf}
	\caption{Past results.}
    \label{fig:eval-ablation-adapter}
\end{figure}




==> fig-eval-adapter-heatmap.tex <==
\begin{figure}[t]
    \includegraphics[width=0.38\textwidth]{figs/eval-heatmap-TC.pdf}
    \caption{Ablation of trained adapters from continuous layer spans. }
    \label{fig:eval-adapter-heatmap}
\end{figure}

% The heatmap shows the relative decrease in validation accuracy to the fully trained adapted model. The y and x axes indicate the first and last layers ablated (inclusive), respectively. The diagonal cells, indicate ablation of a single layer's adapters. The cell in the top-right indicates ablation of all adapters. Cells in the lower triangle are meaningless, and are set to 0\%, the best possible relative performance.




% \begin{figure}[t]
%     \centering
%     \begin{minipage}[b]{0.24\textwidth}
%         \includegraphics[width=1.0\textwidth]{figs/eval-heatmap-TC.pdf}
%         \subcaption{Uniform}
%     \end{minipage}
%     ~
%     \begin{minipage}[b]{0.24\textwidth}
%         \includegraphics[width=1.0\textwidth]{figs/eval-heatmap-ST.pdf}
%         \subcaption{Non-iid}
%     \end{minipage}
%     \caption{Ablation of trained adapters from continuous layer spans. The heatmap shows the relative decrease in validation accuracy to the fully trained adapted model. The y and x axes indicate the first and last layers ablated (inclusive), respectively. The diagonal cells, indicate ablation of a single layer's adapters. The cell in the top-right indicates ablation of all adapters. Cells in the lower triangle are meaningless, and are set to 0\%, the best possible relative performance.}
%     \label{fig:eval-adapter-heatmap}
% \end{figure}



==> fig-eval-adapter-select-cache.tex <==
\begin{figure*}[t]
    \small
    \centering
    \begin{minipage}[b]{0.24\textwidth}
        \includegraphics[width=1.0\textwidth]{figs/eval-adapter-select-cache.pdf}
        \subcaption{TC: \texttt{20NEWS} (uniform)}
    \end{minipage}
    ~
    \begin{minipage}[b]{0.24\textwidth}
        \includegraphics[width=1.0\textwidth]{figs/eval-adapter-select-cache.pdf}
        \subcaption{TC: agnews (niid-label)}
    \end{minipage}
    ~
    \begin{minipage}[b]{0.24\textwidth}
        \includegraphics[width=1.0\textwidth]{figs/eval-adapter-select-cache.pdf}
        \subcaption{TC: ttc (niid-quantity)}
    \end{minipage}
    ~
    \begin{minipage}[b]{0.24\textwidth}
        \includegraphics[width=1.0\textwidth]{figs/eval-adapter-select-cache.pdf}
        \subcaption{ST: onto (niid)}
    \end{minipage}
    ~
    \caption{Introduce on-device activations caching to further accelarate the compuation.}
    % \caption{The performance breakdown of computation and communication time. Note that y-axis is logarithmic.}
    \label{fig:eval-adapter-select-cache}
\end{figure*}

==> fig-eval-adapter.tex <==
\begin{figure*}[t]
    \centering
    \begin{minipage}[b]{0.24\textwidth}
        \includegraphics[width=1.0\textwidth]{figs/eval-adapter.pdf}
        \subcaption{TC: \texttt{20NEWS} (uniform)}
    \end{minipage}
    ~
    \begin{minipage}[b]{0.24\textwidth}
        \includegraphics[width=1.0\textwidth]{figs/eval-adapter.pdf}
        \subcaption{TC: agnews (niid-label)}
    \end{minipage}
    ~
    \begin{minipage}[b]{0.24\textwidth}
        \includegraphics[width=1.0\textwidth]{figs/eval-adapter.pdf}
        \subcaption{TC: ttc (niid-quantity)}
    \end{minipage}
    ~
    \begin{minipage}[b]{0.24\textwidth}
        \includegraphics[width=1.0\textwidth]{figs/eval-adapter.pdf}
        \subcaption{ST: onto (niid)}
    \end{minipage}
    ~
    \caption{Under heterogeneous scenarios, stragglers will bottleneck the training. Computation overhead dominates.}
    % \caption{The performance breakdown of computation and communication time. Note that y-axis is logarithmic.}
    \label{fig:eval-adapter}
\end{figure*}

==> fig-eval-breakdown.tex <==
\begin{figure}[t]
    \centering
    \begin{minipage}[b]{0.24\textwidth}
        \includegraphics[width=1.0\textwidth]{figs/eval-breakdown.pdf}
        \subcaption{DistilBert}
    \end{minipage}
    ~
    \begin{minipage}[b]{0.24\textwidth}
        \includegraphics[width=1.0\textwidth]{figs/eval-breakdown.pdf}
        \subcaption{Bert}
    \end{minipage}
    \caption{Runtime breakdown of training time per batch. Left column: no cached; Right colum: cached.}
    % \caption{The performance breakdown of computation and communication time. Note that y-axis is logarithmic.}
    \label{fig:eval-breakdown}
\end{figure}

==> fig-eval-device-heterogeneity.tex <==
\begin{figure}[t]
    \centering
    \begin{minipage}[b]{0.23\textwidth}
        \includegraphics[width=1.0\textwidth]{figs/eval-device-heterogeneity-30.pdf}
        \subcaption{Client\_num=30}
    \end{minipage}
    ~
    \begin{minipage}[b]{0.23\textwidth}
        \includegraphics[width=1.0\textwidth]{figs/eval-device-heterogeneity-100.pdf}
        \subcaption{Client\_num=100}
    \end{minipage}
    % ~
    % \begin{minipage}[b]{0.13\textwidth}
    %     \includegraphics[width=1.0\textwidth]{figs/eval-device-heterogeneity-1000.pdf}
    %     \subcaption{Client\_num=1000}
    % \end{minipage}
    \caption{Device heterogeneity}
    % \caption{The performance breakdown of computation and communication time. Note that y-axis is logarithmic.}
    \label{fig:eval-device-heterogeneity}
\end{figure}

==> fig-eval-fairness.tex <==
% \begin{figure}[t]
%     \centering
%     \begin{minipage}[b]{0.24\textwidth}
%         \includegraphics[width=1.0\textwidth]{figs/eval-energy-unfair.pdf}
%         \subcaption{Without adaptive}
%     \end{minipage}
%     ~
%     \begin{minipage}[b]{0.24\textwidth}
%         \includegraphics[width=1.0\textwidth]{figs/eval-energy-fair.pdf}
%         \subcaption{Adaptive}
%     \end{minipage}
%     \caption{Without adaptive, those weak devices will compute more and hence consume more energy.}
%     % \caption{The performance breakdown of computation and communication time. Note that y-axis is logarithmic.}
%     \label{fig:eval-fairness}
% \end{figure}

==> fig-eval-performance-distilbert.tex <==
% \begin{figure*}[t]
%     \centering
%     \begin{minipage}[b]{0.24\textwidth}
%         \includegraphics[width=1.0\textwidth]{figs/eval-performance-distilbert-20news.pdf}
%         \subcaption{\texttt{20NEWS}}
%     \end{minipage}
%     ~
%     \begin{minipage}[b]{0.24\textwidth}
%         \includegraphics[width=1.0\textwidth]{figs/eval-performance-distilbert-agnews.pdf}
%         \subcaption{\texttt{AGNEWS}}
%     \end{minipage}
%     ~
%     \begin{minipage}[b]{0.24\textwidth}
%         \includegraphics[width=1.0\textwidth]{figs/eval-performance-distilbert-semeval.pdf}
%         \subcaption{\texttt{SEMEVAL}}
%     \end{minipage}
%     ~
%     \begin{minipage}[b]{0.24\textwidth}
%         \includegraphics[width=1.0\textwidth]{figs/eval-performance-distilbert-onto.pdf}
%         \subcaption{\texttt{ONTONOTES}}
%     \end{minipage}
%     ~
% %    \caption{The time-to-accuracy of \sys and baselines with DistilBERT.}
%         \caption{Time-to-accuracy throughout a training session. NLP model: DistilBERT. \sys{} speeds up model convergence significantly.}    
%     % \caption{The performance breakdown of computation and communication time. Note that y-axis is logarithmic.}
%     \label{fig:eval-performance-distilbert}
% \end{figure*}

% % \begin{table*}[]
% %     \footnotesize
% %     \begin{tabular}{|l|ll|ll|ll|ll|}
% %     \hline
% %              & \multicolumn{2}{c|}{TC (20news)}    & \multicolumn{2}{c|}{TC (agnews)}   & \multicolumn{2}{c|}{TC (semeval)}   & \multicolumn{2}{c|}{ST (onto)}       \\ \hline
% %     Methods & \multicolumn{1}{l|}{Comm.} & Speedup & \multicolumn{1}{l|}{Comm.} & Speedup & \multicolumn{1}{l|}{Comm.} & Speedup & \multicolumn{1}{l|}{Comm.} & Speedup \\ \hline
% %     Origin   & \multicolumn{1}{l|}{26.70} & 1      & \multicolumn{1}{l|}{44.49} & 1.00  & \multicolumn{1}{l|}{260.67} & 1.00  & \multicolumn{1}{l|}{1034.31} & 1.00  \\ \hline
% %     Freeze   & \multicolumn{1}{l|}{7.10}  & 3.76   & \multicolumn{1}{l|}{14.02} & 3.17  & \multicolumn{1}{l|}{105.39} & 2.47  & \multicolumn{1}{l|}{649.47}  & 1.59  \\ \hline
% %     Adaptive & \multicolumn{1}{l|}{0.18}  & 150.40 & \multicolumn{1}{l|}{0.67}  & 66.78 & \multicolumn{1}{l|}{2.63}   & 99.13 & \multicolumn{1}{l|}{33.60}   & 30.78 \\ \hline
% %     \end{tabular}
% %     \caption{Network Traffic Save}
% %     \label{tab:eval-communication}
% %     \end{table*}

==> fig-eval-select-client.tex <==
\begin{figure*}[t]
    \centering
    \begin{minipage}[b]{0.24\textwidth}
        \includegraphics[width=1.0\textwidth]{figs/eval-adapter-select-client.pdf}
        \subcaption{TC: 20news (uniform)}
    \end{minipage}
    ~
    \begin{minipage}[b]{0.24\textwidth}
        \includegraphics[width=1.0\textwidth]{figs/eval-adapter-select-client.pdf}
        \subcaption{TC: agnews (niid-label)}
    \end{minipage}
    ~
    \begin{minipage}[b]{0.24\textwidth}
        \includegraphics[width=1.0\textwidth]{figs/eval-adapter-select-client.pdf}
        \subcaption{TC: ttc (niid-quantity)}
    \end{minipage}
    ~
    \begin{minipage}[b]{0.24\textwidth}
        \includegraphics[width=1.0\textwidth]{figs/eval-adapter-select-client.pdf}
        \subcaption{ST: onto (niid)}
    \end{minipage}
    ~
    \caption{Choosing those devices of similar capcity, we overcome the delimma from stragglers.}
    % \caption{The performance breakdown of computation and communication time. Note that y-axis is logarithmic.}
    \label{fig:eval-adapter-select-client}
\end{figure*}

==> fig-impl.tex <==
\begin{figure}[t]
	\centering
	\includegraphics[width=0.48\textwidth]{figs/impl.pdf}
	\caption{The system architecture of \sys.}
    \label{fig:impl}
\end{figure}


==> recycle/recycle-sec-intro.tex <==
\section{Introduction}\label{sec:intro}

\input{fig-overview}

Transformers/BERT are the SOTA models for ML tasks for its abilities to:
1. obtain good accuracy;
2. generalize to many tasks through fine-tuning.

We envision BERT can serve as a fundamental, important building block for on-device intelligence in near future.
Indeed, an (optimized) BERT can be deployed on devices now, on non-realtime tasks (with a few hundreds ms).

While pre-training is done on large, public dataset, fine-tuning often needs domain-specific, private data. (meaning on-device data, as owned by users of the devices)
Therefore we cannot simply collect raw training data from clients.
Instead, we can use federated learning.

( -- Felix's writing below -- )

With recent rise of transformers, NLP tasks show compelling use cases on client devices. 
Examples include ... auto completion, conversational agents, ...

\paragraph{The paradigm of FedNLP}
A central motivation: training samples (language contents) are generated by end users continually; 
owned by the users and distributed over client devices. 

As a result, the de facto paradigm to deploy NLP models on the edge (/smartphones)... is through 
fine-tuning of large pre-trained models ... 

Specifically, two core techniques underpinning the deployment paradigm: 

(1) Fine-tuning (for downstream tasks of a given domain, e.g. sentiment analysis of restaurant reviews). 
Reason: diverse downstream language tasks (e.g. QA, classification, translation, generation. impractical to deploy models for each); 
newly emerged domains (driven by apps, language topics, contents) 
and datasets (user-generated language contents; user preference, styles); 
in many cases, such datasets are unavailable ahead of deployment time. 

(2) FL. Users want to preserve privacy of their language materials. 
Do not upload (give away) the data to the cloud for training. 
FL is being recognized as the common practice~\cite{lin2021fednlp,bonawitz2019towards}
Client devices collaborate to fine-tune a global model using their respective data without giving away the data.  
How many rounds ... each round the cloud select client devices to participate ... 

In this paper, we follow prior work~\cite{lin2021fednlp} and refer to the above paradigm (on-device fine-tuning of NLP models, in a federated fashion) as ``FedNLP''. 

\paragraph{Characterization of overhead} 
Despite the established algorithm framework, the FedNLP overhead is high, 
resulting in prohibitively slow model convergence. 
For instance, ... will take a few days. 
Due to the large sizes of NLP models, the convergence delay is much longer than, e.g. vision models under federated settings (often XXX hours). 

To motivate system building, 
we first characterize the overhead over a suite of XXX benchmarks. 
\begin{comment}
It reveals two challenges:
1. Scalability issue: directly fine-tuning the model, even with several layers freezed, is not parameter efficient;
2. Cost issue: on-device fine-tuning (training) is prohibitively resource-hungry, e.g., memory, time, network, and energy.
\end{comment}
 
As we have measured, .... twofold: 
(1) high communication cost. A problem long known to FL (each round participating devices download the updated model). 
Exacerbated by the large NLP model size (transformer-based). 
(2) high on-device computation cost. 

Towards practical FedNLP, there is a large efficiency gap to bridge (reducing overhead from days ?? to hours? minutes??)
% the overhead has to be reduced by at least 

\paragraph{A framework}
We present a system framework for on-device fine-tuning of NLP models (FedNLP). 
The framework integrates a suite of algorithm and system components in a novel fashion. 

\begin{itemize}
\item 
Adapters. 
An emerging algorithmic modules for deep neural networks. 
As per-layer, small add-on to a neural network (NN), adapters become the only tunable modules in the NN, allowing freezing the NN's other parameters in the fine-tuning process. 

While adapters are previously used for ... we identify them as key building blocks for FedNLP. 
We are the first applying adapters to federated learning. 
Significant reduction in the tunable parameters. Much less data to exchange (communication cost).


\mwx{Does adapter have math foundation?}

\item 
On-device cache of activations. (feature maps?) 
FL typically runs multiple/many rounds (e.g. XXX) to converge. 
In particular suitable to FL, where the untuned bottom layers are only executed once across N rounds. 
The cache can be preserved on disk instead of memory. 
In subsequent rounds (each round with a set of updated top layers from the cloud), 
the untuned bottom layers do not need to be touched (both forward pass and backward pass). 
Note: the new model may update bottom layers \textit{below} the cached activations, simply because those layers may have been tuned on other clients. 
To handle this case, the client either invalidates the cache and recomputes from the bottom layer, or caches activations at every layer (expensive).
\mwx{Make recomputation latency hidden under other stages.}


\item 
Variable tuning depth. 
Fine tuning deeper layers results in higher accuracy (helps convergence rate), but in return requires much higher resource. 
More capable devices tune deeper layers; and vice versa. 
This is done via device selection by the cloud. 
Aggregation: per round. 
\mwx{A system model: each device can finetune X--Y layers based on its capacity and status (hard constraint: memory). Per round, there is a set of devices available per round. What to select? Considering the device heterogeneity and convergence status.}
(Each round: the same number of adapters/layers) 

\item 
A scheduling algorithm (or a planner) at the cloud side, 
the goal is to reduce the convergence delay. 
at a convergence point (target accuracy for the global model), what device and depth of adapters to select? 
The framework reduces the costs of communication and computation by at least one order of magnitude. 
\end{itemize}


As we will show, each component is indispensable. 
All things combined, the convergence time is reduced to XXX seconds.  
For the first time, we show that on-device NLP fine-tuning is practical. 



Therefore, we propose a system to tackle the above challenges.
It retrofits two existing techniques:
1. adapters;
2. secure outsourcing.

What are our unique novelty?

\paragraph{Contributions}

\begin{itemize}
\item A first-of-its-kind measurement study (characterization) of FedNLP ... on client devices. 
\item A novel system that integrates adapters, variable tuning depth, and activation cache. 
\item Experiments show fast convergence and accuracy
\end{itemize}

==> sec-design-overview.tex <==
\subsection{Overview}

\sys is a federated learning scheme for NLP finetuning tasks with the primary goal to optimize the time-to-accuracy during training.
It is designed with following principles.

\xzlNote{these are more likes goals than ``principles''}

\begin{itemize}[leftmargin=*]
\item \sys minimizes the efforts from developers in adapting a pre-trained model for a specific downstream task.
\item \sys considers each finetuning task to be unseen, therefore its technique does not rely on any historical knowledge of finetuning on the same downstream task.
\item \sys does not impose any constraint on the client selection~\mwx{refs} or training data sampling~\mwx{refs} strategies, making it compatible with a mass of recent FL system literature.
\end{itemize}


\xzlNote{Move to S2.3? implications}

\textbf{Challenges}
\sys deals with two major challenges.
First, as demonstrated in $\S$\ref{sec:measurement}, federated learning of a modern NLP model is slow due to the considerable amount of time spent on data transmission and local training per round.
Simply freezing part of the model brings only modest improvement.
It requires architecture-level redesign or adaptation from the vanilla NLP model.

\xzlNote{This is to justify dynamism/adaptation, right? If so, we should just say so. And in addition to diverse tasks, talk about diverse devices/resources/etc}
Second, a notable characteristic of NLP scenario is that there are abundant, hetergeneous downstream tasks.
The training data distribution to such tasks is not known ahead of time.
As we will show in $\S$\ref{sec:design:scheduler}, different tasks demand different adaptation to the NLP model to achieve a good convergence performance.
Exploring different model adaptations on the fly often imposes huge resource and time waste, which violates the design principle of \sys.


\xzlNote{below seems unneeded}
\textbf{\sys techniques}
To address the first challenge, \sys first borrows the concept of \textit{adapters} designed for parameter-efficient continuous learning~\mwx{refs} ($\S$\ref{sec:design:adapter}).
By freezing the whole original pre-trained model but only updating the inserted adapters, \sys can significantly reduce the data exchanged among devices and central server.
\sys further employs an activation caching technique to reduce the on-device training computations by exploiting the opportunity that most model parameters are sustained across FL rounds ($\S$\ref{sec:design:cache}).
To tackle the second challenge, \sys employs a lightweight trial-and-error approach to automatically adapt the models to the downstream tasks ($\S$\ref{sec:design:scheduler}).

==> sec-eval-bandwidth.tex <==
/subsection

==> sec-eval-dataset.tex <==
\subsection{Tasks and Datasets}


==> tab-bandwidth-heterogeneity.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table*}[]
  \footnotesize
    \begin{tabular}{@{}|c|l|ll|ll|ll|ll|@{}}
    \toprule
    \multicolumn{1}{|l|}{\textbf{}} &
      \textbf{} &
      \multicolumn{2}{c|}{\textbf{TC (20news)}} &
      \multicolumn{2}{c|}{\textbf{TC (agnews)}} &
      \multicolumn{2}{c|}{\textbf{TC (semeval)}} &
      \multicolumn{2}{c|}{\textbf{ST (onto)}} \\ \midrule
    \multicolumn{1}{|l|}{\textbf{Bandwidth}} &
      \textbf{Methods} &
      \multicolumn{1}{l|}{acc=0.8} &
      acc=0.7 &
      \multicolumn{1}{l|}{acc=0.9} &
      acc=0.8 &
      \multicolumn{1}{l|}{acc=0.8} &
      acc=0.7 &
      \multicolumn{1}{l|}{f=0.8} &
      f=0.7 \\ \midrule
     &
      Origin &
      \multicolumn{1}{l|}{41.68} &
      7.95 &
      \multicolumn{1}{l|}{13.19} &
      1.55 &
      \multicolumn{1}{l|}{76.98} &
      16.34 &
      \multicolumn{1}{l|}{305.71} &
      48.18 \\ \cmidrule(l){2-10} 
     &
      Freeze &
      \multicolumn{1}{l|}{16.92} &
      2.38 &
      \multicolumn{1}{l|}{4.66} &
      0.07 &
      \multicolumn{1}{l|}{32.36} &
      7.77 &
      \multicolumn{1}{l|}{199.23} &
      27.29 \\ \cmidrule(l){2-10} 
    \multirow{-3}{*}{1} &
      Adaptive &
      \multicolumn{1}{l|}{{\color[HTML]{FE0000} 2.72}} &
      {\color[HTML]{FE0000} 0.25} &
      \multicolumn{1}{l|}{{\color[HTML]{FE0000} 0.94}} &
      {\color[HTML]{FE0000} 0.01} &
      \multicolumn{1}{l|}{{\color[HTML]{FE0000} 3.54}} &
      {\color[HTML]{FE0000} 1.01} &
      \multicolumn{1}{l|}{{\color[HTML]{FE0000} 45.77}} &
      {\color[HTML]{FE0000} 6.63} \\ \midrule
     &
      Origin &
      \multicolumn{1}{l|}{21.73} &
      4.10 &
      \multicolumn{1}{l|}{6.83} &
      0.84 &
      \multicolumn{1}{l|}{40.30} &
      8.63 &
      \multicolumn{1}{l|}{159.63} &
      25.31 \\ \cmidrule(l){2-10} 
     &
      Freeze &
      \multicolumn{1}{l|}{9.52} &
      1.36 &
      \multicolumn{1}{l|}{2.62} &
      0.05 &
      \multicolumn{1}{l|}{17.56} &
      4.18 &
      \multicolumn{1}{l|}{107.76} &
      14.83 \\ \cmidrule(l){2-10} 
    \multirow{-3}{*}{2} &
      Adaptive &
      \multicolumn{1}{l|}{{\color[HTML]{FE0000} 2.58}} &
      {\color[HTML]{FE0000} 0.22} &
      \multicolumn{1}{l|}{{\color[HTML]{FE0000} 0.88}} &
      {\color[HTML]{FE0000} 0.01} &
      \multicolumn{1}{l|}{{\color[HTML]{FE0000} 3.13}} &
      {\color[HTML]{FE0000} 0.99} &
      \multicolumn{1}{l|}{{\color[HTML]{FE0000} 43.03}} &
      {\color[HTML]{FE0000} 6.42} \\ \midrule
     &
      Origin &
      \multicolumn{1}{l|}{11.91} &
      2.22 &
      \multicolumn{1}{l|}{3.64} &
      0.44 &
      \multicolumn{1}{l|}{21.78} &
      4.65 &
      \multicolumn{1}{l|}{85.55} &
      13.53 \\ \cmidrule(l){2-10} 
     &
      Freeze &
      \multicolumn{1}{l|}{5.97} &
      0.82 &
      \multicolumn{1}{l|}{1.61} &
      0.03 &
      \multicolumn{1}{l|}{10.04} &
      2.50 &
      \multicolumn{1}{l|}{61.24} &
      8.41 \\ \cmidrule(l){2-10} 
    \multirow{-3}{*}{4} &
      Adaptive &
      \multicolumn{1}{l|}{{\color[HTML]{FE0000} 2.34}} &
      {\color[HTML]{FE0000} 0.22} &
      \multicolumn{1}{l|}{{\color[HTML]{FE0000} 0.82}} &
      {\color[HTML]{FE0000} 0.01} &
      \multicolumn{1}{l|}{{\color[HTML]{FE0000} 3.06}} &
      {\color[HTML]{FE0000} 0.94} &
      \multicolumn{1}{l|}{{\color[HTML]{FE0000} 40.92}} &
      {\color[HTML]{FE0000} 6.12} \\ \midrule
     &
      Origin &
      \multicolumn{1}{l|}{6.86} &
      1.19 &
      \multicolumn{1}{l|}{2.09} &
      0.27 &
      \multicolumn{1}{l|}{12.54} &
      2.61 &
      \multicolumn{1}{l|}{48.88} &
      7.70 \\ \cmidrule(l){2-10} 
     &
      Freeze &
      \multicolumn{1}{l|}{4.18} &
      0.55 &
      \multicolumn{1}{l|}{1.16} &
      0.02 &
      \multicolumn{1}{l|}{6.29} &
      1.57 &
      \multicolumn{1}{l|}{{\color[HTML]{FE0000} 38.50}} &
      {\color[HTML]{FE0000} 5.28} \\ \cmidrule(l){2-10} 
    \multirow{-3}{*}{8} &
      Adaptive &
      \multicolumn{1}{l|}{{\color[HTML]{FE0000} 2.14}} &
      {\color[HTML]{FE0000} 0.19} &
      \multicolumn{1}{l|}{{\color[HTML]{FE0000} 0.77}} &
      {\color[HTML]{FE0000} 0.01} &
      \multicolumn{1}{l|}{{\color[HTML]{FE0000} 3.04}} &
      {\color[HTML]{FE0000} 0.84} &
      \multicolumn{1}{l|}{39.33} &
      5.77 \\ \bottomrule
    \end{tabular}
    \caption{BandWidth Heterogeneity. Device: Hybrid}
    \label{tab: eval-bandwidth-heterogenity}
    \end{table*}

==> tab-eval-adaptive-ablation <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[]
    \footnotesize
    \begin{tabular}{@{}ccccc@{}}
    \toprule
    \textbf{OntoNote} & \textbf{Origin} & \textbf{Optim-Freeze} & \textbf{Dyna-Adapter}             & \textbf{Vanilla Adapter} \\ \midrule
    Time (h)              & 304.21          & 197.36                & \cellcolor[HTML]{FD6864}40.69 & 54.60                    \\
    Speedup        & $1.00\times$            & $1.54\times$                   & \cellcolor[HTML]{FD6864}$7.48\times$   & $5.57\times$                      \\ \bottomrule
    Network(G)	& 517.16 	& 324.74 	& 16.80 	& 22.94 \\ \bottomrule
    \end{tabular}
    \caption{Dynamic Adapter VS Vanilla Adapter. Time \& Speedup when arriving at the target metric $f1\_score=0.8$.}
    \label{tab:adaptive-ablation}
    \end{table}

==> tab-eval-device-heterogeneity <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table*}[]
  \footnotesize
    \begin{tabular}{@{}|c|l|ll|ll|ll|ll|@{}}
    \toprule
    \multicolumn{1}{|l|}{\textbf{}} &
      \textbf{} &
      \multicolumn{2}{c|}{\textbf{TC (20news)}} &
      \multicolumn{2}{c|}{\textbf{TC (agnews)}} &
      \multicolumn{2}{c|}{\textbf{TC (semeval)}} &
      \multicolumn{2}{c|}{\textbf{ST (onto)}} \\ \midrule
    \multicolumn{1}{|l|}{\textbf{Device}} &
      \textbf{Methods} &
      \multicolumn{1}{l|}{acc=0.8} &
      acc=0.7 &
      \multicolumn{1}{l|}{acc=0.9} &
      acc=0.8 &
      \multicolumn{1}{l|}{acc=0.8} &
      acc=0.7 &
      \multicolumn{1}{l|}{f=0.8} &
      f=0.7 \\ \midrule
     &
      Origin &
      \multicolumn{1}{l|}{40.75} &
      7.70 &
      \multicolumn{1}{l|}{12.83} &
      1.51 &
      \multicolumn{1}{l|}{75.16} &
      16.00 &
      \multicolumn{1}{l|}{298.22} &
      47.09 \\ \cmidrule(l){2-10} 
     &
      Freeze &
      \multicolumn{1}{l|}{15.52} &
      2.12 &
      \multicolumn{1}{l|}{4.19} &
      0.07 &
      \multicolumn{1}{l|}{30.79} &
      7.40 &
      \multicolumn{1}{l|}{189.73} &
      25.99 \\ \cmidrule(l){2-10} 
    \multirow{-3}{*}{TX2} &
      Adaptive &
      \multicolumn{1}{l|}{{\color[HTML]{FE0000} 1.28}} &
      {\color[HTML]{FE0000} 0.12} &
      \multicolumn{1}{l|}{{\color[HTML]{FE0000} 0.44}} &
      {\color[HTML]{FE0000} 0.01} &
      \multicolumn{1}{l|}{{\color[HTML]{FE0000} 1.68}} &
      {\color[HTML]{FE0000} 0.47} &
      \multicolumn{1}{l|}{{\color[HTML]{FE0000} 22.01}} &
      {\color[HTML]{FE0000} 3.19} \\ \midrule
     &
      Origin &
      \multicolumn{1}{l|}{51.16} &
      9.66 &
      \multicolumn{1}{l|}{16.11} &
      1.89 &
      \multicolumn{1}{l|}{94.37} &
      20.09 &
      \multicolumn{1}{l|}{374.43} &
      59.12 \\ \cmidrule(l){2-10} 
     &
      Freeze &
      \multicolumn{1}{l|}{30.11} &
      4.12 &
      \multicolumn{1}{l|}{8.14} &
      0.14 &
      \multicolumn{1}{l|}{46.17} &
      11.09 &
      \multicolumn{1}{l|}{284.53} &
      38.98 \\ \cmidrule(l){2-10} 
    \multirow{-3}{*}{RPI} &
      Adaptive &
      \multicolumn{1}{l|}{{\color[HTML]{FE0000} 15.16}} &
      {\color[HTML]{FE0000} 1.40} &
      \multicolumn{1}{l|}{{\color[HTML]{FE0000} 5.25}} &
      {\color[HTML]{FE0000} 0.07} &
      \multicolumn{1}{l|}{{\color[HTML]{FE0000} 19.45}} &
      {\color[HTML]{FE0000} 5.46} &
      \multicolumn{1}{l|}{{\color[HTML]{FE0000} 258.52}} &
      {\color[HTML]{FE0000} 37.89} \\ \midrule
     &
      Origin &
      \multicolumn{1}{l|}{43.38} &
      8.25 &
      \multicolumn{1}{l|}{13.83} &
      1.65 &
      \multicolumn{1}{l|}{80.17} &
      16.96 &
      \multicolumn{1}{l|}{316.15} &
      49.99 \\ \cmidrule(l){2-10} 
     &
      Freeze &
      \multicolumn{1}{l|}{19.31} &
      2.63 &
      \multicolumn{1}{l|}{5.33} &
      0.09 &
      \multicolumn{1}{l|}{34.90} &
      8.23 &
      \multicolumn{1}{l|}{212.91} &
      29.07 \\ \cmidrule(l){2-10} 
    \multirow{-3}{*}{Straggler} &
      Adaptive &
      \multicolumn{1}{l|}{{\color[HTML]{FE0000} 4.96}} &
      {\color[HTML]{FE0000} 0.47} &
      \multicolumn{1}{l|}{{\color[HTML]{FE0000} 1.84}} &
      {\color[HTML]{FE0000} 0.02} &
      \multicolumn{1}{l|}{{\color[HTML]{FE0000} 6.45}} &
      {\color[HTML]{FE0000} 1.68} &
      \multicolumn{1}{l|}{{\color[HTML]{FE0000} 79.63}} &
      {\color[HTML]{FE0000} 11.55} \\ \bottomrule
    \end{tabular}
    \caption{Device Heterogeneity. BW: 1MB/s}
    \label{tab: eval-device-heterogenity}
    \end{table*}

==> tab-motivation-freezing.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[t]
\footnotesize
\begin{tabular}{|l|r|r|rr|}
\hline
\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}Freezing\\ Layers\end{tabular}}} & \multicolumn{1}{l|}{\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}Training\\ Time (sec)\end{tabular}}}} & \multicolumn{1}{l|}{\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}Updated\\Params (MB)\end{tabular}}}} & \multicolumn{2}{c|}{\textbf{Accuracy}} \\ \cline{4-5} 
 & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{\textbf{Dataset1}} & \multicolumn{1}{l|}{\textbf{Dataset2}} \\ \hline
E & 100 & 100 & \multicolumn{1}{r|}{0.80} & 0.80 \\ \hline
E+T$_0$ & 100 & 100 & \multicolumn{1}{r|}{0.80} & 0.80 \\ \hline
E+T$_{0-1}$ & 100 & 100 & \multicolumn{1}{r|}{0.80} & 0.80 \\ \hline
E+T$_{0-2}$ & 100 & 100 & \multicolumn{1}{r|}{0.80} & 0.80 \\ \hline
E+T$_{0-3}$ & 100 & 100 & \multicolumn{1}{r|}{0.80} & 0.80 \\ \hline
E+T$_{0-4}$ & 100 & 100 & \multicolumn{1}{r|}{0.80} & 0.80 \\ \hline
E+T$_{0-5}$ & 100 & 100 & \multicolumn{1}{r|}{0.80} & 0.80 \\ \hline
\end{tabular}
\caption{The training performance with different freezing point of DistilBERT. ``E'' is embedding layer and ``T$_{x-y}$'' means the $x_{th}$ to $y_{th}$ transformer layers. Training time is obtained on RPI-3B.}
\label{tab:motivation-freezing}
\end{table}
